LodeStar: Maritime Radar Descriptor for Semi-Direct Radar Odometry

Maritime radars are prevalently adopted to capture the vessel's omnidirectional data as imagery. Nevertheless, inherent challenges persist with marine radars, including limited frequency, suboptimal resolution, and indeterminate detections. Additionally, the scarcity of discernible landmarks in the vast marine expanses remains a challenge, resulting in consecutive scenes that often lack matching feature points. In this context, we introduce a resilient maritime radar scan representation LodeStar, and an enhanced feature extraction technique tailored for marine radar applications. Moreover, we embark on estimating marine radar odometry utilizing a semi-direct approach. LodeStar-based approach markedly attenuates the errors in odometry estimation, and our assertion is corroborated through meticulous experimental validation.

==> result_table.tex <==
%\begin{table*}
%\resizebox{\linewidth}{!}{
%\begin{tabular}{c|c|cccc|c} 
%\hline
%\multirow{2}{*}{\textbf{Criteria}} & \multirow{2}{*}{\textbf{Approach}} &\multicolumn{4}{c|}{\textbf{Mulran Dataset}} & {\textbf{Oxford Dataset}}\\ 

% & & \textbf{DCC}  & \textbf{KAIST} & \textbf{Riverside} & \textbf{Sejong} & \textbf{2019-01-16 to 2019-01-18}\\ 
%\hline\hline
% & Raplace(Proposed) & \textbf{0.932} & \textbf{0.930} & \textbf{0.971} & \textbf{0.906} & %\textbf{0.949} \\
%\textbf{F1 Score} & Scan Context & 0.867 & 0.899 & 0.802 & 0.819 & 0.679\\
%& PointNetVLAD & 0.xxx & 0.xxx & 0.xxx & 0.xxx & 0.xxx\\
%\cline{1-7}
%& Raplace(Proposed) & \textbf{0.978} & \textbf{0.984} & \textbf{0.995} & \textbf{0.969} & %\textbf{0.959} \\
%\textbf{AUC} & Scan Context & 0.952 & 0.978 & 0.915 & 0.929 & 0.773\\
%& PointNetVLAD & 0.xxx & 0.xxx & 0.xxx & 0.xxx & 0.xxx  \\

%\end{tabular}}
%\caption{Global Localization Results.}\label{tab:gl_result}
%\end{table*}

\begin{table}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|ccc}
\multicolumn{2}{c}{\textbf{Dataset}}                                                    & \textbf{Method} & \textbf{AUC}   & \textbf{F1 Score} \\ \hline\hline
\multicolumn{1}{c|}{\multirow{12}{*}{MulRan}} & \multirow{3}{*}{DCC}       & ScanContext     & 0.952          & 0.867             \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\  
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.978} & \textbf{0.932}    \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multirow{3}{*}{KAIST}     & ScanContext     & 0.978          & 0.899    \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\  
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.984} & \textbf{0.930}             \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multirow{3}{*}{Riverside} & ScanContext     & 0.915          & 0.802             \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\  
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.995} & \textbf{0.971}    \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multirow{3}{*}{Sejong}    & ScanContext     & 0.929          & 0.819             \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.969} & \textbf{0.906}    \\ \hline
\multicolumn{2}{c|}{\multirow{3}{*}{Oxford}}                     & ScanContext     & 0.773          & 0.679             \\  
\multicolumn{2}{c|}{}                                              & PointNetVlad    &                &                   \\ 
\multicolumn{2}{c|}{}                                          & RaPlace         & \textbf{0.959} & \textbf{0.949}    \\  \hline
\end{tabular}
}
\caption{Global Localization Results}\label{tab:gl_result}
\end{table}

==> result_table_comb.tex <==
\begin{table}[t!]
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{cc|c|cc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset}}}                    & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Global Localization}}       \\
\multicolumn{2}{c|}{}                                                     &                                  & \multicolumn{1}{c}{\textbf{AUC}}   & \textbf{F1 Score} \\ \hline \hline
\multicolumn{1}{c|}{\multirow{8}{*}{MulRan}} & \multirow{2}{*}{DCC}       & SC                               & \multicolumn{1}{c}{0.952}          & 0.867             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.978}} & \textbf{0.932}    \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{KAIST}     & SC                               & \multicolumn{1}{c}{0.978}          & 0.899             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.984}} & \textbf{0.930}    \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Riverside} & SC                               & \multicolumn{1}{c}{0.915}          & 0.802             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.995}} & \textbf{0.971}    \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Sejong}    & SC                               & \multicolumn{1}{c}{0.929}          & 0.819             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.969}} & \textbf{0.906}    \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Oxford}} & \multirow{2}{*}{19-01-16}  & SC                               & \multicolumn{1}{c}{0.773}          & 0.679             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.959}} & \textbf{0.949}    \\ \hline
\end{tabular}
}
\caption{Global Localization Results}\label{tab:gl_result}
\end{table}

==> result_table_pr.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{cc|c|cc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset}}}                    & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Single Session}}\\
\multicolumn{2}{c|}{}                                                     &                                  & \multicolumn{1}{c}{\textbf{AUC}}   & \textbf{F1 Score}\\ \hline \hline
\multicolumn{1}{c|}{\multirow{8}{*}{MulRan}} & \multirow{2}{*}{DCC}       & R-SC                               & \multicolumn{1}{c}{0.801}          & 0.679            \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.843}} & \textbf{0.735}   \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{KAIST}     & R-SC                               & \multicolumn{1}{c}{0.819}          & \textbf{0.786}   \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.881}} & 0.781            \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Riverside} & R-SC                               & \multicolumn{1}{c}{0.944}          & 0.862            \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.959}} & \textbf{0.897}   \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Sejong}    & R-SC                               & \multicolumn{1}{c}{0.904}          & 0.830            \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.924}} & \textbf{0.858}   \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Oxford}} & \multirow{2}{*}{19-01-16}  & R-SC                               & \multicolumn{1}{c}{0.545}          & 0.534            \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.595}} & \textbf{0.543}   \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{19-01-18}  & R-SC                               & \multicolumn{1}{c}{0.826}          & \textbf{0.773}   \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.827}} & 0.734            \\ \hline
\end{tabular}
}
\caption{Intra-session Place Recognition Results}\label{tab:pr_result}
%\vspace{-5mm}
\end{table*}
